Memory-Based Model Editing at Scale

Even the largest neural networks make errors, and once-correct predictions can become invalid as the world changes. Model editors make local updates to the behavior of base (pre-trained) models to inject updated knowledge or correct undesirable behaviors. Existing model editors have shown promise, but also suffer from insufficient expressiveness: they struggle to accurately model an edit's intended scope (examples affected by the edit), leading to inaccurate predictions for test inputs loosely related to the edit, and they often fail altogether after many edits. As a higher-capacity alternative, we propose Semi-Parametric Editing with a Retrieval-Augmented Counterfactual Model (SERAC), which stores edits in an explicit memory and learns to reason over them to modulate the base model's predictions as needed. To enable more rigorous evaluation of model editors, we introduce three challenging language model editing problems based on question answering, fact-checking, and dialogue generation. We find that only SERAC achieves high performance on all three problems, consistently outperforming existing approaches to model editing by a significant margin. Code, data, and additional project information will be made available at https://sites.google.com/view/serac-editing.

==> figures/tex/multi_model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/imgs/multi_model.png}
    \caption{Applying the same editor to many models. Left shows editing all T5 models with a single editor (t5-small used for early stopping during training). Right shows editing various models in the GPT-2 family with a single editor (distilGPT-2 used for early stopping during training). For both model families, a single {\name} editor is able to provide consistent edits for all models within the family. \textbf{PLACEHOLDER; THESE NUMBERS AREN'T REAL AND ARE TOTALLY MADE UP}}
    \label{fig:multi-model}
\end{figure}

==> history/abs.tex <==

%%%%%%%%%%%%%%%%%
%%%%% Abs v4 %%%%%
%%%%%%%%%%%%%%%%%
\cm{This leaps from world state being dynamic in first sentence to models having errors in the 3rd sentence. I think you probably do want to mention both cases, but more symmetrically. You also spend 3 sentences on this scene setting whereas you might think one or two is sufficient: Large pre-trained neural networks harbor errors and beyond that the state of the world continually changes with elections and death. It is therefore highly desirable to model editors that can quickly and precisely apply local updates to model behavior.}
World knowledge is dynamic: heads of state change every few years and medical best practices are updated based on new research. Methods for quickly and precisely editing deployed machine learning models to reflect new knowledge are therefore valuable. \textit{Model editors} make such local updates to the behavior of base (pre-trained) models to correct errors or modulate behavior. While existing model editors have shown promising results, they also have shortcomings that limit their practical utility. In particular, existing approaches struggle to accurately capture the scope of an edit, leading to inaccurate predictions when test inputs are loosely related to the edit, and sometimes fail altogether when many edits are needed. In this work, we propose an explicit memory-based approach to model editing, which not only addresses both of the challenges above, but also produces an editor that can be reused across multiple base models. To enable more rigorous evaluation of model editors, we also introduce three new challenging language model editing problems based on question answering, fact-checking, and dialogue generation, finding that the memory-based model editor produces edits that generalize better and scale to a greater number of edits than existing approaches. \cm{Delete ``new'' -- it's hard to introduce something pre-existing!}
%% Can't include specific numbers until we have the experiments, but will add later



%%%%%%%%%%%%%%%%%
%%%%% Abs 3 %%%%%
%%%%%%%%%%%%%%%%%
The ability to make fast, targeted edits to a neural network's behavior would enable an otherwise-accurate model to remain deployed when specific facts about the world change, such as when a new head of state is elected or a medical best practice is updated. 
%%CF.1.22: I like Antoine's suggested start. Though, I would tweak the phrasing to: "World knowledge is dynamic: e.g. heads of state change every few years, and medical best practices are updated based on new research. Thus, we need the ability to quickly and precisely edit models to reflect new knowledge.
\textit{model editors} make such local updates to the behavior of base (pre-trained) models to correct errors or modulate behavior. While existing model editors have shown promising results, they also have shortcomings that limit their practical utility. In particular, existing approaches fail when many edits are needed and cause spurious predictions from the edited model for inputs related to the edit example. 
%%CF.1.22: potential revision: existing approaches struggle when many edits are needed and also struggle to accurately capture the scope of an edit, leading to inaccurate predictions when test inputs are loosely related to the edit. 
In this work, we propose an explicit memory-based approach to model editing, which not only addresses both of the challenges above, but can also be re-used across multiple base models.
%%CF.1.22: but also produces an editor that can be reused across multiple base models.
To enable more rigorous evaluation of model editors, we also introduce three new challenging language model editing problems based on question answering, fact-checking, and dialogue generation, finding that the memory-based model editor produces edits that generalize better and scale to a greater number of edits than existing approaches.
%% Can't include specific numbers until we have the experiments, but will add later


%%%%%%%%%%%%%%%%%
%%%%% Abs 2 %%%%%
%%%%%%%%%%%%%%%%%
Model editors locally modify the behavior of a base (pre-trained) model to correct errors or modulate behavior, often using only a single example to do so. 
%%✓CF.1.17: I think it would be helpful to have some additional motivation here, to explain why you might want to locally modify a model. (e.g. knowledge becoming out-of-date, etc). While this is apparent to you, it will not be apparent to your reader.
%%CF.1.17: Also be careful with wording like "using only a single example". Learned model editors rely on an entire dataset of edits for training, not just a single example.
Existing model editors directly update the parameters of the base model in order to modify their behavior, but recent works have noted that the effectiveness of these approaches drops significantly when multiple edits are applied, model degradation is measured using inputs related to the edit example,
%%✓CF.1.17: The above is not at all easy to parse or understand, even when reading multiple times. I also think that the point about directly updating the parameters of the base model, since this bit of info isn't crucial at this point. I might rephrase the whole sentence to: "While recent approaches have shown promising results, they also have a number of drawbacks that severely limit their practical utility. These limitations include the ability to handle large batches of edits and the ability to accurately make predictions on inputs near the edit example. In this work, we introduce..."
or edits are required to generalize beyond simple paraphrases of the edit example. In this work, we introduce an expressive new memory-based approach to model editing, which improves on existing methods in each of these circumstances and allows an editor to be re-used across multiple base models, unlike existing methods. 
%%CF.1.17: Your sentences are quite long. It is often better for readability to break it up into shorter sentences, covering only one idea per sentence. e.g. "In this work, we propose an explicit memory-based approach to model editing. This memory-based editor not only addresses both of the challenges above, but can also be re-used across multiple base models." Note how by revision is two sentences, but is actually a bit shorter than the original sentence.
To enable more rigorous evaluation of model editors, we also introduce three new challenging language model editing problems based on question answering, fact-checking, and dialogue generation, finding that the memory-based model editor produces edits that generalize better and scale to a greater number of edits than existing approaches.
%%CF.1.17: If you can give more specific numbers to the above, that would be nice

%%%%%%%%%%%%%%%%%
%%%%% Abs 1 %%%%%
%%%%%%%%%%%%%%%%%
Model editors aim to enable fast, targeted adjustments to a deployed neural network’s behavior without retraining. However, in this paper, we find that gradient-based editors are insufficiently expressive to make successful model edits in a variety of realistic settings. We propose a gradient-free, semi-parametric approach to editing that learns to correct a trained model’s predictions using an explicit memory of edits. We show that this approach enjoys significant advantages over past model editors in terms of both edit reliability and computational efficiency as model size, number of edits, or edit difficulty increases.

==> history/experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% v1 %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%


\section{Experiments}
\label{sec:expts}
We study the behavior of model editors along several axes of difficulty of the model editing problem, including a) overall performance, especially on hard in-scope and hard out-of-scope examples; b) capacity to apply multiple simultaneous edits; and c) ability to use explicit edit descriptors that are not input-output pairs. In addition, we provide an error analysis of the memory-based editor a study the effects of varying the scope classifier architecture.
%%CF.1.25: technically it's only an ablation if you remove something from the algorithm

% We want to highlight all of:
% \begin{enumerate}
%     \item Batched/sequential edits: An editor trained with single edits generalizes for free to 125 edits with basically no drop in performance
%     \item Generalization and scaling across models: One editor gives the same edit performance on e.g. t5-small, t5-large, and t5-xl with no further training/tuning; this means we can scale to “infinitely” large models
%     \item Solving implications: The implications dataset is solvable for t5large at $\sim$91\% accuracy (MEND basically can’t make any progress on implications using t5)
%     \item Reducing overgeneralization: Drawdown on adversarial examples is significantly reduced (by maybe half?) by using hard negatives during training, with edit success still higher than MEND
%     \item Low complexity: The implementation is super simple
%     \item Interpretable errors: edit failures can be decomposed into either scope classifier errors (incorrect inference of equivalence neighborhood) or replacement errors (incorrect counterfactual reasoning)
%     \item Iterative editing: if an edit leads to overgeneralization, negative examples can just be added to the edit cache to mitigate these, making edit refinement much easier (\textbf{may be hard without human evals})
% \end{enumerate}

\subsection{Experimental Settings}

Our experiments use a combination of existing and novel editing settings, including question-answering, fact-checking, and conversational dialogue. See Table~\ref{tab:hard-pos-neg} for data samples from each setting. The QA-hard and FC settings are motivated by the desire to better test a model editor's capacity to handle harder in-scope and out-of-scope examples. The ConvSent setting is intended to both evaluate generation models on a problem more tied with real-world usage as well as explore the possibility of applying edits that are not simply input-output pairs.
%%CF.1.25: Feel free to add any more motivation as needed. There were other issues with the previous benchmarks too
%%EM done

\textbf{QA \& QA-hard.} The QA setting uses the zsRE question-answering problem introduced by \citet{Cao2021EditingFK}. We use this dataset as a starting point of reference to connect our evaluations with prior work. For the QA-hard setting, we generate harder in-scope examples that test logically entailed facts (\rawstring{$\ze =$ Who is the UK PM? Boris Johnson $\rightarrow$ $\xtest =$ Where is Boris Johnson the PM?}) or true/false questions (\rawstring{$\xtest =$ True or False: Theresa May is the UK PM}) using automated techniques \citep{demszky2018transforming,ribeiro2019red}. Crucially, both types of hard in-scope examples will have labels that differ from the edit example, requiring some non-trivial reasoning over the edit descriptor to produce the correct post-edit output. In addition, to generate hard out-of-scope examples for an edit input $\xe$, we selectively sample from training inputs $x$ that have high semantic similarity with $\xe$, measured as having a high cosine similarity between their embeddings as computed by a pre-trained semantic embedding model \texttt{all-MiniLM-L6-v2} \citep{reimers-2019-sentence-bert}. For both QA and QA-hard, we use a T5-large model (770m parameters; \citet{2020t5}) fine-tuned on the Natural Questions dataset \citep{kwiatkowski2019natural,roberts2020knowledge} as the base model.

\textbf{FC.} We introduce a new FC setting using the VitaminC fact verification dataset \citep{schuster-etal-2021-get} to assess an editor's ability to update an out-of-date fact-checking model's when presented with updated information about the world. VitaminC contains over 400,000 evidence-claim-page-label tuples $(e_i, c_i, p_i, l_i)$ where the label $l_i$ is 1 if the evidence entails the claim, -1 if it contradicts the claim, or 0 if neither. The dataset was gathered from Wikipedia revisions in the first half of 2020. To convert VitaminC into an editing dataset, we first use $e_i$ as each edit descriptor $\ze[i]$. Using $C$ to denote the set of \textit{all} claims in the VitaminC dataset and the function $\beta(p_i)=\{c_j : p_j = p_i\}$ as the set of claims from page $p_i$, we define in-scope and out-of-scope examples as
\begin{equation*}
    I(\ze[i]),\;O(\ze[i]) = \begin{cases}
        \{(c_i, 1)\},\phantom{\varnothing} C \setminus \beta(p_i) & \text{if}\;l_i = 1 \\
        \{(c_i, 0)\},\phantom{\varnothing} C \setminus \beta(p_i) & \text{if}\;l_i = 0 \\
        \varnothing,\phantom{\{(c_i, 0)\}} \{c_i\} & \text{if}\;l_i = -1,
    \end{cases}
\end{equation*}

%%CF.1.25: I find this pretty difficult to understand because there is a lot of notation. Though, not sure if I have a good way to address that. 
%%EM: moved notation before block.
%%CF.1.25: Perhaps the bigger issue is that it's pretty weird to have this define both I and O, especially since the RHS doesn't seem to output two things. why not just have two lines , one for I and one for O?
%%CF.1.25: also FYI, I(\ze) should be I(\ze; \editdataset)
. For $l_i \in \{0,1\}$, we have `easy' out-of-scope examples sampled uniformly from all claims. For $l_i=-1$, we have hard out-of-scope examples, as these claims are still closely semantically related to the evidence. As a base model, we use the BERT-base model trained by \citet{Cao2021EditingFK} on the June 2017 Wikipedia dump in the FEVER dataset \citep{Thorne18Fever}.
%%CF.1.25: "Wikipedia dump" seems a bit informal though I'm not familiar with the terminology in NLP
%%EM: This is the terminology used in the original FEVER paper; it's fairly common in NLP

\input{figures/tex/multi_model}

\textbf{ConvSent.} Our final new dataset is focused on generation models. The ConvSent editing problem assesses a model editor's ability to edit the sentiment of a dialogue agent on a particular topic without affecting its generations when prompted on other topics. We gather a list of 15,000 non-numeric entities from zsRE and 989 noun phrases from GPT-3 \citep{brown2020language} (e.g., \rawstring{ghost hunting} or \rawstring{the dangers of artificial intelligence}) for a total of 15,989 topics. For each entity, we sample 10 noisy positive sentiment completions and 10 noisy negative sentiment completions from the 3B parameter BlenderBot model \citep{roller2021recipes}, using a template such as \rawstring{Tell me a \{negative/positive\} opinion on \_\_\_.}. We then use a pre-trained sentiment classifier \citep{heitmann2020} based on RoBERTa \citep{liu2019robustly} to compute more accurate sentiment labels for each completion. For this task, edit descriptors take the simple form of \rawstring{Topic: \_\_\_ Sentiment: \{Positive/Negative\}}, rather than a prompt/completion pair. We define $I(\ze)$ with a manually collected set of templates such as \rawstring{What do you think of \_\_\_?} or \rawstring{Tell me your thoughts on \_\_\_.}, using the prompts formed with different templates but the same entity as in-scope examples. We define $O(\ze; \editdataset)$ as all examples generated from entities \textit{other} than the one used in $\ze$. We use the smaller 90m parameter BlenderBot model \citep{roller2021recipes} as the base model for this experiment, as it is currently state-of-the-art in dialog. %\footnote{Note that we could use any dialogue model as a base model for this experiment, but we use BlenderBot as it is currently state-of-the-art in dialogue.}

\textbf{Comparison algorithms.} 
We perform experiments evaluating a variety of existing approaches to model editing in a variety of difficult editing settings. We consider gradient-based editors, fine-tuning on the edit example (\textbf{FT}), editable neural networks (\textbf{ENN}; \citet{Sinitsin2020Editable}), KnowledgeEditor (\textbf{KE}; \citet{Cao2021EditingFK}), and model editor networks using gradient decomposition (\textbf{MEND}; \citet{mitchell2021fast}), as well as a cache+lookup baseline \textbf{LU} \footnote{We cache the average hidden state of $\xe$ computed by $\basemodel$, returning $\ye$ for new inputs $x'$ with hidden state less than $\delta$ from the hidden state of $\xe$ and $\basemodel(x')$ otherwise}. We also consider a `retrieve-and-prompt' ablation \textbf{RP} that uses a scope classifier identical to the one in the memory-based editor to retrieve a relevant edit example from the cache if there is one, but uses the base model $\basemodel$ rather than the counterfactual model $\rep$ to make the final prediction.

\input{figures/tex/multi_edit}

\subsection{Evaluating model editors on challenging tasks}

\subsection{Re-using model editors across models}

In this section, we demonstrate that the memory-based editor can be trained independently from any particular base model, leading to significant practical advantages. The most powerful model editors described in past works must be re-trained or re-fit for each new model they are intended to edit \citep{Sinitsin2020Editable,Cao2021EditingFK,mitchell2021fast,anon2021moving}. Further, these editors require access to the internal activations and gradients of $\basemodel$, leading to computational costs of training the editor to scale with the size of $\basemodel$ \citep{mitchell2021fast}. In contrast, the memory-based editor can be directly applied without modification to edit multiple models, and the computational costs of training are \textit{constant} with respect to base model size. Figure~\ref{fig:multi-model} shows the results. A single memory-based T5-editor shows consistently high edit success and low drawdown across 4 different T5 models, while a single memory-based GPT-2-editor shows similarly high edit success and low drawdown across 4 different GPT-2 models.


\subsection{Making many edits}

While past research in model editing has largely focused on single model edits, some works have noted that successfully applying multiple edits either as a batch \citep{mitchell2021fast} or in sequence \citep{hase2021language} is significantly more difficult than the single edit setting. In this section, we conduct experiments to understand how editor behavior changes as the number of sequentially-applied edits increases. Figure~\ref{fig:multi-edit} shows the results. Gradient-based editors exhibit near-monotonic decrease in their ability to both successfully update model predictions and prevent model degradation.

% \subsection{Undergeneralization in model editors}

% Past work has shown that existing model editors tend to make relatively superficial edits, failing to generalize to \textit{hard positives}, post-edit inputs that require reasoning about information entailed by an edit. See Table~\ref{tab:hard-pos-neg} for examples of hard positives for various datasets. In this experiment, we train each model editor with and without hard positives (the suffix `+' indicates the algorithm was trained with hard positives), evaluating with hard positives in both cases. Table~\ref{tab:undergeneralization} shows the results. {\name} is the only editor expressive enough to leverage hard positives during training; other algorithms exhibit significantly degraded performance on \textit{easy} positives when training with hard positives. In other words, they underfit the more difficult training distribution containing hard positives.

% \subsection{Overgeneralization in model editors}
% Basically same as undergeneralization, but looking at hard negatives instead of hard positives

\subsection{Error Analysis}
\input{tables/error_decomp}
One advantage of the memory-based editor is the ability to decompose editor errors into classification errors and counterfactual prediction errors. Table~\ref{tab:decomp} shows the performance breakdown across editor components (scope classifier and counterfactual model) and data sub-split (all data, hard positives, hard negatives, etc.) when applying zsRE question-answering edits to a T5-large model.

\subsection{Ablations}
We perform a set of experiments to understand how classifier architecture impacts the behavior of the memory-based editor. Using the QA-hard and FC tasks with $k=10$ edits, we compare the cross-attention-based (Cross) and dense embedding-based (Embed) classifier using both distilBERT (\textbf{D}; \citep{Sanh2019DistilBERTAD}) and BERT-base (\textbf{B}; \citep{devlin2019bert}) as the backbone model. The results are shown in Table~\ref{tab:ablations}. Unsurprisingly, both increasing the size of the classifier and using cross-attention instead of dense-embeddings is helpful for editor performance. Cross-attention is especially useful for the FC experiment, which is possibly due to the commonness of quantities in the VitaminC dataset; producing fixed-length sequence embeddings that reliably capture the difference between \rawstring{There have been 105,000 coronavirus deaths in the United States} and \rawstring{There have been 111,000 coronavirus deaths in the United States} may be very difficult. In this case, late fusion approaches \citep{khattab2020colbert} may be useful in increasing expressiveness while limiting compute requirements.

==> history/fig1.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/png/fig1.png}
    \caption{\textit{Overview of {\name}}. 
    When evaluating new test inputs $x, x'$ after several edit examples $\{x^i_e, y^i_e\}$ have been applied, we first embed the test inputs and edit examples with $\feat$ to find the most relevant (closest in embedding space) edit example for each test input. If the nearest edit example is within a (learned) threshold distance to the test input, we return the output of the counterfactual model $\rep$, which conditions on both the test input and nearest neighbor edit example, instead of the base model.
    }
    \label{fig:method-overview}
\end{figure}

==> history/intro.tex <==


%%%%%%%%%%%%%%%##%%
%%%%% Intro 2 %%%%%
%%%%%%%%%%%%%##%%%%


Large neural networks, notably language models, are typically deployed as static artifacts, whose behavior is difficult to modify during deployment without re-training \citep{lazaridou2021mind}. While prepending either manually-written or automatically-retrieved prompts to the input can sometimes be effective for modulating behavior \citep{brown2020language}, model predictions often do not update to reflect the content of the prompts \citep{lewis2020retrieval}. However, in order to respond to changes in the world 
%%CF.1.22: to respond to changes in the world
(e.g., new heads of state or evolving public sentiment on a particular topic) or correcting for instances of underfitting or overfitting of original training data,
%%CF.1.22: in the original training data?
the ability to quickly make targeted updates to model behavior after deployment is desirable. To address this need, \textit{model editing} is an emerging area of research that aims to enable fast, data-efficient updates to a pre-trained \textit{base model}'s behavior for only a small region of the domain, without damaging model performance on other inputs of interest \citep{Sinitsin2020Editable,zhu2020modifying,sotoudeh2019correcting,Cao2021EditingFK,dai2021knowledge,mitchell2021fast,hase2021language,anon2021moving}.

A popular approach to model editing involves learnable model editors, which are trained to predict updates to the weights of the base model that ultimately produce the desired change in behavior \citep{Sinitsin2020Editable,Cao2021EditingFK,mitchell2021fast,hase2021language}. While these approaches have shown promise, in line with recent work \citep{hase2021language}, we find that existing methods produce model updates that fail to discriminate between entailed and non-entailed facts
%%CF.1.22: in scope and out of scope?
%%EM: Thinking about leaving this as-is because we haven't introduced that terminology yet
and cannot handle large numbers of edits. Further, existing editors coupling 
%%CF.1.22: couple or "existing editors are trained for a particular base model"
the model editor and base model, and thus the model editor must be re-trained for each new base model to be edited. This coupling also leads to computational costs of model editor training that scale with the size of the base model, which can prove unwieldy for even for models an order of magnitude smaller than the largest deployed language models \citep{mitchell2021fast}. In aggregate, existing model editors still have shortcomings regarding edit performance, compute efficiency, and ultimately practicality. We hypothesize that these shortcomings are related to the reliance of existing methods on the \textit{gradient} of the edit example label with respect to the pre-edit model parameters. Leveraging the observation in \citet{csordas2021are} that for two related inputs to a neural network, the two corresponding subsets of the model's parameters responsible for its predictions may be nearly disjoint sub-networks.
%%CF.1.22: The above is not a complete sentence. (i.e. "leveraging the observation that the two corresponding subsets" is not a sentence)
The gradient for one example (e.g., the edit example) may therefore contain almost no information about how to update parameters that are needed to make predictions for distant, but related examples.
%%CF.1.22: I would shorten this above part to a single sentence rather than three. The intro is already quite long (especially considering that you will be adding stuff to the end of the last paragraph), and this info seems like it is helpful for motivation, but not critical especially given how long-winded it is.

\input{figures/tex/fig1}

Building on the hypothesis that gradients are an impoverished signal for model editing, we propose a gradient-free \textit{memory-based} approach to model editing. This approach `wraps' a black-box base model with an explicit cache of applied edit examples
%%CF.1.22: an explicit cache of used-provided edit examples
(arbitrary utterances)
%%CF.1.22: I don't think this adds anything
and a small auxiliary \textit{classifier} and \textit{counterfactual model}. Rather than making model edits in parameter space, this editor simply stores edit examples in the cache without modifying the base model. When a post-edit test input is received, the classifier determines if any edit in the cache is relevant. If an edit is classified as relevant, the counterfactual model uses the test input and edit example together to predict the test input label under the counterfactual world described by the edit. If no edit examples are deemed relevant to the test input, the base model simply predicts the test input label. See Figure~\ref{fig:method-overview} for an example of both cases. Intuitively, this approach delegates the sub-problems of \textit{when} the model's predictions should change to the classifier and \textit{how} they should change to the counterfactual model. While existing methods attempt to solve both of these problems implicitly in base model parameter space by transforming the raw edit example gradient, the memory-based approach solves each with its own small but expressive neural network, reducing interference between these two sub-problems. Further, the classifier reduces interference between edits by predicting relevance scores for each pair of (test input, edit cache example) separately. Finally, access to the base model is not longer necessary with this decoupling\footnote{We only need its tokenization.}, enabling the trained editor to be applied to multiple models without modification and decoupling the cost of editor training from base model size.

Our primary contribution is a framework for memory-based editing that shows far better performance and computational efficiency than existing methods. We also introduce three new editing problems, based on the tasks of question-answering, fact-checking, and dialogue generation, which are far more challenging than existing editing benchmarks. Our experiments indicate that the memory-based editor consistently outperforms past approaches to model editing and enables successful model editing in more realistic scenarios than existing methods.
%%% Will add more specific numbers when we have them

%%CF.1.22: Overall, this looks much better than the last version that I looked at!



%%%%%%%%%%%%%%%##%%
%%%%% Intro 1 %%%%%
%%%%%%%%%%%%%##%%%%

Large neural networks, notably language models, are typically deployed as static artifacts, whose behavior is difficult to modify during deployment without re-training \citep{lazaridou2021mind}.
%%CF.1.17: what about prompting? that seems to be a bit of an elephant in the room here. though, maybe it's fine to not address here.
However, the ability to quickly make targeted updates to model behavior after deployment is useful for a variety of purposes, including responding to changes in the state of the world (e.g., new heads of state or evolving public sentiment on a particular topic) or correcting for instances of underfitting or overfitting of original training data.
%%CF.1.17: I would flip this around, and start by saying the issues with static models and then say that making targeted updates would be useful for addressing it.
Model editing is an emerging area of research that aims to create \textit{model editors},
%%CF.1.17: model editing aims to create model editors? The above is more long winded than it needs to be. The full sentence is also quite long.
which enable fast, data-efficient\footnote{Often using only a single example}
%%CF.1.17: Footnotes break up the flow a lot. I wouldn't recommend it in this case. Keep in mind that readability is as important if not more important than trying to include all of these details.
updates to a pre-trained \textit{base model}'s behavior for only a small region of the domain, without damaging model performance on other inputs of interest \citep{Sinitsin2020Editable,zhu2020modifying,sotoudeh2019correcting,Cao2021EditingFK,dai2021knowledge,mitchell2021fast,hase2021language,anon2021moving}.

% \textbf{[summarize issues with gradient-based editors]} 
The most successful approaches to model editing generally use learnable model editors \citep{Sinitsin2020Editable,Cao2021EditingFK,mitchell2021fast,hase2021language},
%%CF.1.17: Saying that they are the most successful seems like it may be unnecessarily controversial/subjective. Overall success can be measured in a number of ways, and some people may view the need to train model editors as a large flaw. It's also not necessary to make a statement about what is most successful. You can just say "Learned model editors approach the editing problem by learning to predict updates to the weights of the base model that ultimately produce the desired change in behavior~\cite{}." 
which are trained to predict updates to the weights of the base model that ultimately produce the desired change in behavior. While these approaches have shown promise, in line with recent work \citep{hase2021language}, we find that their performance degrades significantly when evaluated on editing problems that are more aligned with real-world conditions. Specifically, existing methods fail to reliably produce model parameter updates that can discriminate between entailed and non-entailed facts, and parameter updates for different examples exhibit interference when many simultaneous or sequential edits are needed. 
%%CF.1.17: You can phrase this more cleanly and concisely as: Specifically, existing methods produce updates that cannot reliably discriminate between entailed and non-entailed facts and cannot handle large numbers of edits.
Further, learning to estimate parameter updates directly has the conceptual drawback of coupling the model editor and base model, which induces both a requirement to re-train the model editor for each new base model to be edited and computational costs of model editor training that scale with the size of the base model \citep{mitchell2021fast}.
%%CF.1.17: the phrasing of the last part could be improved
Ultimately, these factors lead to significant computational costs for training model editors for multiple large base models. 
%%CF.1.17: I would make this last sentence a bit broader in scope, more towards the entire paragraph. e.g. "Ultimately, these factors lead to significant drawbacks in terms of performance, compute, and practicality."

\input{figures/tex/fig1}

% \textbf{[briefly describe semi-parametric editor]} 
%%CF.1.17: Can you guide the reader towards the answer instead of just stating the answer? As written, this first sentence does not make it clear how the method addresses the issues raised before, making this first sentence a bit more confusing.
As an alternative, we propose a \textit{memory-based} approach to model editing, which stores edits (input/output pairs) as they are received in an explicit cache, treats the base model as a black box, and ultimately decouples the model editor from the base model.
%%CF.1.17: The above has too much info in one sentence.
The editor learns a \textit{classifier} that predicts if a post-edit model input is relevant to any existing edit example; if an edit in the cache is deemed relevant, the cached edit and model input are both passed to a learned \textit{counterfactual model} that learns to make counterfactual predictions for a given model input, conditioned on the information in the edit. If no edit examples are deemed relevant to the new model input, the input is simply passed to the base model. We describe a training procedure for both the classifier and counterfactual model that do not require access to the base model at all, only its tokenization, enabling the trained editor to be applied to multiple models without modification and decoupling the cost of editor training from base model size. 
%%CF.1.17: The above paragraph doesn't do anything to describe how or why the new approach addresses the three challenges. It only says that it does not require access to the base model, but doesn't explain how/why, and it doesn't say anything about the other two challenges. Explaining this intuition is super important, since intuition and new ideas/concepts are often more valuable than new methods themselves, since it's the intuition and ideas that drive the field forward. (unless you are expecting people to use the method as is and not the ideas in future work, which seems unlikely to me)
%%CF.1.17: I would leave the below to the last paragraph when you talk about the experimental results, so that this paragraph can focus entirely on the method.
To evaluate the generalization and scalability of the memory-based editor, we introduce three new editing problems, including question-answering, fact-checking, and dialogue generation. We find that these editing problems are far more challenging than existing benchmarks for editing.

% \textbf{[summarize benefits/novelties]} 
%%CF.1.17: I would recommend putting this in paragraph form, starting with stating the main contribution (e.g. a framework/method for memory-based editing), then discussing some of the secondary contributions like the description of the challenges and the new suite of challenging editing tasks, and then finally discussing the experimental results.
%%CF.1.17: I think that the current list doesn't have enough detail on the experimental results, and it also puts these contributions on equal footing, which isn't quite accurate.
Our primary contributions are:
\begin{compactenum}
    \item Three new challenging editing tasks, which evaluate models for sequence classification, transduction, and generation
    \item The description of the problematic behaviors of \textit{over-generalization} and \textit{under-generalization} behavior in existing model editors
    \item The memory-based model editor, which demonstrates better generalization behavior and far better computational efficiency than existing model editors
    %%CF.1.17: how much better, and on what kinds of problems? This description is not very precise, and is also rather generic -- many papers could say that they get better generalization and efficiency than existing methods. What is more interesting is -- how much is the improvement, what are the points of comparison, what are the ablations, and what do these experiments tell us about the model editing problem?
\end{compactenum}

% \begin{compactenum}
%     \item The computational cost of training {\name} is \textbf{constant} with respect to the size of the model to be edited.
%     \item {\name} can be trained \textbf{once} and immediately deployed without modification to edit \textbf{many} models.\footnote{For language models, the counterfactual model and base model must share the same tokenization.}
%     \item {\name} can make many \textbf{simultaneous} or \textbf{sequential} edits to a model with essentially no drop in performance.
%     \item {\name} is expressive enough to learn to make \textbf{deep model edits} that generalize beyond simple paraphrases of the edit provided.
%     \item {\name} can \textbf{distill} the semi-parametric edited model back into the original pre-edit model's parameters, avoiding a constantly-growing cache of model edits.
% \end{compactenum}

==> history/method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% v1 %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%


\section{A Memory-Based Model Editor}
\label{sec:method}
To motivate a model editor that does not modify the base model parameters, we note the observation by \citet{csordas2021are} that neural networks `over-specialize' their parameters to individual inputs. That is, for two related inputs to a neural network, the two corresponding subsets of the model's parameters responsible for its predictions may have very little overlap, or even be disjoint. The gradient for one example (e.g., an edit descriptor $\editpair$) may therefore contain little useful information for updating the parameters responsible for predictions for distant, but related examples (e.g., $\xtest$ or $\xloc$). In light of the potential shortcomings of gradient-based model editors, we propose the memory-based (or, semi-parametric) approach model editing, which directly reasons over the explicit content of the edit descriptors, rather than relying a derivative quantity such as a gradient.

The memory-based approach to model editing is intuitively simple, wrapping the base model with an explicit cache of edits, an edit scope classifier, and a counterfactual model that `overrides' the base model when necessary. After applying several edits, the `wrapped' model makes a prediction for a new input in two steps. First, the classifier estimates the probability that the new input falls into the scope of each cached edit example. If the classifier's in-scope probability is greater than 0.5 for any edit, the edit giving the highest probability is retrieved, and the counterfactual model's prediction conditioned on both the new input and edit is returned. Otherwise, the base model's prediction is returned. This procedure is described in Figure~\ref{fig:method-overview} and is described more formally in the next section.

After applying several edits $\edits=\{\ze[i]\}$, the `wrapped' model makes a prediction for a new input $\xunk$ in two steps. First, the classifier estimates $\alpha^i = P(\xunk \in \scope{\ze[i]})$, the probability that $\xunk$ falls into the scope of the cached edit $\ze[i]$ for all $i$ up to $|\edits|$. We define $i^* = \argmax_i \alpha^i$, the most likely edit example to contain $\xunk$ in its scope.
% Assuming that equivalence neighborhoods are disjoint\footnote{We could generalize this to a $k$-disjointness property, in which an equivalence neighborhood overlaps with only up to $k-1$ other neighborhoods; however, for existing benchmarks, the ($1$-)disjointness property suffices.}, $\xtest$ may fall into the equivalence neighborhood of no more than one of the edit examples in $\edits$. 
Second, if $\alpha^{i^*} > 0.5$, the prediction from the counterfactual model, conditioned on both $\xunk$ and $\ze[i^*]$, is returned; otherwise $\basemodel(x)$ is returned. This procedure is described in Figure~\ref{fig:method-overview} and is described more formally in the next section.

\subsection{{\fullname}}

{\name} is essentially a semi-parametric model of the form $\semimodel(\xtest, \basemodel, \phi, \psi, \edits)$ (we abbreviate as just $\semimodel(\xtest)$) that produces predictions in the output space $\mathcal{Y}$, where $\edits$ is a set of variable size. {\name} contains two key components, a \textit{classifier} and a \textit{counterfactual model}. The classifier $\cls(\xtest, \xe, \ye) : \inp \times (\inp \times \out) \rightarrow [0, 1]$ estimates the probability that an input $\xtest$ falls within the equivalence neighborhood of edit example $(\xe, \ye)$. The counterfactual model $\rep(\xtest, \xe, \ye) : \inp \times (\inp \times \out) \rightarrow \out$ predicts what the label for $\xtest$ would be under the counterfactual world described by $(\xe, \ye)$. The classifier's output is computed as\footnote{This parameterization can be interpreted as producing the pdf of an \textit{unnormalized} multivariate Gaussian centered at $\rep([\xe;\ye])$ with diagonal covariance $\frac{1}{\gamma}$, evaluated at $\rep(\xtest)$.}
\begin{equation}
    \cls(\xtest, \xe, \ye) = \exp\left[-\gamma \|\feat(x) - \feat([\xe; \ye])\|^2_2\right]
\end{equation}
where $\feat$ is a learned embedding function parameterized by $\phi$, $\text{sim}$ is cosine similarity, $\gamma$ is a learned scaling parameter, and $[\xe; \ye]$ is the concatenation of the edit input and target sequences. The counterfactual model $\rep$ is simply a small sequence model (such as GPT-2-small or T5-small) that prepends the edit example $[\xe; \ye]$ to the input $\xtest$.

\textbf{Forward pass (test time).} When presented with an input $\xtest$ at test time, {\name} computes the forward pass as
\begin{equation}
    \semimodel(\xtest) = 
    \begin{cases}
        \basemodel(\xtest) & \beta < 0.5 \\
        \rep(\xtest, \xe^{i^*}, \ye^{i^*}) & \beta \ge 0.5
    \end{cases}
\end{equation}
where $i^* = \argmax_i \cls(\xtest, \xe^i, \ye^i)$, the index of the most relevant edit example, and $\beta = \cls(\xtest, \xe^{i^*}, \ye^{i^*})$, the similarity score of the most relevant edit example. If $\edits$ is empty, we simply set $\semimodel(\xtest) = \basemodel(\xtest)$.
\subsection{Training}
Similarly to past work \citep{Cao2021EditingFK,mitchell2021fast,hase2021language}, {\fullname} is trained using a dataset of the form $\editdata = \{(\xe,\ye,\xloc,\xtest,\ytest)\}$, where $\ze$ is the edit descriptor, $\xloc$ is the negative example (whose label should not change after editing) used to learn a precise editor, and $(\xtest, \ytest)$ is a sample from $N(\xe, \ye)$ used to learn a general editor. In some cases, each training tuple may contain a hard negative $\hxloc$ and/or a hard positive $(\hxtest, \hytest)$. We train the classifier and counterfactual model separately, both with supervised learning.

The \textbf{classifier} $\cls$ is trained to predict whether an input $x$ falls within the equivalence neighborhood $N(\xe, \ye)$ of a particular edit example. Therefore, the classifier is trained to minimize average binary cross entropy loss over the training dataset $\editdata$, assigning label 1 to $(\xtest, \xe, \ye)$ and $(\hxtest, \xe, \ye)$ and label 0 to $(\xloc, \xe, \ye)$ and $(\hxloc, \xe, \ye)$. The \textbf{counterfactual model} $\rep$ is trained to minimize the negative log likelihood of $\ytest$ given $[\xe; \ye; \xtest]$ and $\hytest$ given $[\xe; \ye; \hxtest]$ on average over $\editdata$.

The classifier loss is given as\footnote{We omit terms using hard positives and negatives for brevity, but when hard positives or negatives are available, they are added to the loss in the same way as other positives and negatives.}
\begin{multline}
\ell(\phi) = -\frac{1}{|\editdata|}\sum_j \log g_\phi(\xtest, \xe^j, \ye^j)\;+ \\
         \log (1 - g_\phi(\xloc, \xe^j, \ye^j)).
\end{multline}
The counterfactual loss is similarly
\begin{equation}
\ell(\psi) = -\frac{1}{|\editdata|}\sum_j \log p_\psi(\ytest | \xe, \ye, \xtest)
\end{equation}
where in a slight abuse of notation $p_\psi(\cdot | \xe, \ye, \xtest)$ is the probability distribution over label sequences given the inputs and parameters $\psi$.

Failures of \textit{precision} are entirely attributable to the classifier; negative examples do not appear in the loss function for the counterfactual model. Failures of \textit{generality} may be due to failures of either the classifier (false negative) or the counterfactual model (evaluating the counterfactual incorrectly when the classifier correctly detects a positive pair).


% In contrast to past gradient-based model editors, {\name} can be trained \textit{completely independently from the models it will edit}. In other words, a single model editor can be trained and immediately applied to both a deployed distilGPT-2 model with $\sim$80 million parameters and a full-sized GPT-3 model over three orders of magnitude larger with no modification (assuming they both use the same tokenization). Perhaps more importantly, we have decoupled the computational demands of training the model \textit{editor} from the scale of the model it will eventually edit, which is of great practical significance.

==> history/old_tables/generality.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{clccccccc|ccc}
        \toprule
        & Metric & FT & MEND & MEND+ & ENN & ENN+ & KE & KE+ & {\name} & {\name}+ & MEM+ no $\rep$ \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-small (90M)} \\ zsRE}} & ES & & & & & & & & & \\
        & ES-hard & & & & & & & & & \\
        & DD & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-large (770M)} \\ zsRE}} & ES & & & & & & & & & \\
        & ES-hard & & & & & & & & & \\
        & DD & & & & & & & & & \\
        \midrule
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2-med. (330M)} \\ LeapOfThought}} & ES & & & & & & & & & \\
        & ES-hard & & & & & & & & & \\
        & DD & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2 (1.4B)} \\ LeapOfThought}} & ES & & & & & & & & & \\
        & ES-hard & & & & & & & & & \\
        & DD & & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \caption{Evaluating the \textit{generality} of various model editors. ES shows overall edit success averaged over all positives (including hard positives as well as easier semantically-equivalent rephrases); ES-hard shows edit success on \textit{only} hard positives. {\name} is the only method to effectively produce edits that generalize; gradient-based editors (MEND, ENN, KE) significantly underfit the edit training distribution, which contains examples of hard positives.}
    \label{tab:undergeneralization}
\end{table*}

==> history/old_tables/generalization.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{clccccccc|ccc}
        \toprule
        & Metric & FT & MEND & MEND+ & ENN & ENN+ & KE & KE+ & {\name} & {\name}+ & MEM+ no $\rep$ \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-small (90M)} \\ zsRE}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-large (770M)} \\ zsRE}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2-med. (330M)} \\ WikiData5m}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2 (1.4B)} \\ WikiData5m}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \caption{Evaluating the generalization behavior of various model editors, including hard positives and hard negatives. The `+' suffix indicates the method was trained with hard negatives. {\name} is best able to leverage hard negatives mined during training to reduce drawdown without reducing edit success, while other methods see edit success decline when hard negatives are used during training. We report both average drawdown (DD) on all negatives and drawdown only on hard negatives (DD-hard).}
    \label{tab:overgeneralization}
\end{table*}

==> history/old_tables/precision.tex <==
\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{clccccccc|ccc}
        \toprule
        & Metric & FT & MEND & MEND+ & ENN & ENN+ & KE & KE+ & {\name} & {\name}+ & MEM+ no $\rep$ \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-small (90M)} \\ zsRE}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{T5-large (770M)} \\ zsRE}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2-med. (330M)} \\ WikiData5m}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{GPT-2 (1.4B)} \\ WikiData5m}} & ES & & & & & & & & & \\
        & DD & & & & & & & & & \\
        & DD-hard & & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \caption{Evaluating the \textit{precision} of various model editors, specifically to hard negatives. The `+' suffix indicates the method was trained with hard negatives. {\name} is best able to leverage hard negatives mined during training to reduce drawdown without reducing edit success, while other methods see edit success decline when hard negatives are used during training. We report both average drawdown (DD) on all negatives and drawdown only on hard negatives (DD-hard).}
    \label{tab:overgeneralization}
\end{table*}

==> history/problem.tex <==

%%%%%%%%%%%%%%%##%%
%%%%% Problem v2 %%%%%
%%%%%%%%%%%%%##%%%%

We consider the problem of editing a base model $\basemodel$ using an \textit{edit descriptor} $\ze$ describing how the edited model $\editedmodel$ should change its behavior. The edit descriptor may be a concatenated input-output pair $\editpair$ \rawstring{Who is the UK PM? Boris Johnson} 
%%CF.1.23: I think it would probably be a good idea to introduce notation for the input-output pair too, at the very least since you use such notation in figure 1
or an arbitrary utterance \rawstring{Change sentiment on vaccines to be positive.}
%%CF.1.23: I might suggest picking a more mundane example here and leave this to the qualitative results, since the implications of this example (and the reverse of this example) are thought-provoking in a way that distracts the reader from the writing. You'll also have more space to discuss the implications shortly after the experiments, whereas you generally won't have an opportunity to discuss implications in the technical sections.
describing the desired change in model behavior. We can regard the former type of edit descriptor implicit (as the desired change in model behavior must be inferred from the example) and the latter explicit.

In most cases, applying an edit with descriptor $\ze$ should impact model predictions for a large number of inputs. 
%%CF.1.23: "for a large number of inputs that are within the scope of the edit example"? That would allow you to introduce the terminology informally before describing it formally
In the UK example above, the edited model's predictions should change for rephrases of the edit descriptor input as well as for inputs asking about logically-entailed facts like \rawstring{Boris Johnson is the PM of where?} or \rawstring{True or False: Theresa May is the UK PM}. Thus we refer to the set of inputs whose true label is affected by the edit as the \textit{scope} of an edit $\scope{\ze}$. An edit is \textit{successful} if the edited model adheres to the behavior defined by $\ze$ for \textit{in-scope} inputs. An edit is \textit{well-scoped} if model behavior on \textit{out-of-scope} inputs is left unchanged\footnote{We might consider a successful edit as one with high recall and a well-scoped edit as one with high precision, with regards to the input examples for which the edited model behaves as desired.}. If an in-scope input requires some non-trivial reasoning to deduce its label from the edit example, we call it a hard in-scope input.
%%CF.1.23: how about a "hard in-scope example"? I like that a bit better than input here, because the label is part of what makes it hard.
If an out-of-scope input is closely semantically related to the edit example, we call it a hard out-of-scope input.
%%CF.1.23: same comment
In the setting when $n$ edits $\edits = \{\ze[i]\}$ are applied, either in sequence or simultaneously in a batch, we define $\scope{\edits} = \cup_i \scope{\ze[i]}$ to be the union of the individual edit scopes.
%%CF.1.23: I think the below deserves its own paragraph, since it is unrelated to what is discussed above, and is pretty important. I would also suggest putting this info about the training dataset of edits before talking about in-scope/out-of-scope, since it is a core part of the problem statement, whereas the in-scope/out-of-scope is simply defining auxiliary terminology.
To train a model editor, we assume access
%%CF.1.23: I would phrase this more as part of the problem rather than an added assumption, since it is a core part of the problem.  e.g. "Model editors are trained using a dataset of training edits that are representative of the edits that we expect users to provide at test time." (Also, I think it would be worth generally describing the problem in English fully before introducing notation)
to a dataset $\editdata =\{\ze, \xtest, \ytest, \xloc\}$
%%CF.1.23: I would change the notation for \xloc to reflect the out-of-scope terminology. (maybe x_oos?)
of edits describing the types of desired edits, where $\xtest$ is an in-scope test input,
%%CF.1.23: I would avoid the terminology "test input" for examples in the training edit dataset.
$\ytest$ is its corresponding label, and $\xloc$ is an out-of-scope input.
%%CF.1.23: seems like you are missing a \yloc?

%%CF.1.23: It's weird to have one paragraph header in the section (akin to how it is weird to have one subsection in a section). Revise?
\textbf{Evaluation.} Based on the notions of \textit{successful} and \textit{well-scoped} edits, we use the metrics of edit success (\textbf{ES}) and drawdown (\textbf{DD}) to evaluate a model editor.
%%CF.1.23: following prior work?
Intuitively, ES measures similarity between the edited model behavior and the \textit{desired} edited model behavior for in-scope inputs, while DD measures disagreement between the pre-edit and post-edit model for out-of-scope inputs. High ES and low DD is desirable, with ES of one and DD of zero being perfect editor performance.
%%CF.1.23: The below is a bit weird because you are moving from a general definition of the problem to something that is much more specific to the experiments. I think it would be good to have some sign-posting to say something along the lines of "The specific ways of measuring of edit success and drawdown depend on the application domain; hence, we will outline two example instantiations of these metrics next."

For \textbf{question-answering} and \textbf{fact-checking} tasks, we define ES as simply the average exact-match agreement between the edited model and true labels for in-scope inputs:
\begin{equation}
    \mathbf{ES_{ex}}(\ze) \triangleq \frac{1}{|\scope{\ze}|}\sum_{x' \in \scope{\ze}} \mathbbm{1}\{\editedmodel(x') = \ye[x']\}
\end{equation}
where $\ye[\xtest]$ is the desired label for $\xtest$ under the edit $\ze$.
We define drawdown similarly as
\begin{equation}
    \mathbf{DD_{ex}}(\ze,O) \triangleq \frac{1}{|O(\ze)|}\sum_{x' \in O(\ze)} \mathbbm{1}\{\editedmodel(x') \neq \basemodel(x')\}
\end{equation}
%%CF.1.23: If you are going to use notation for O, then it would be worth defining it earlier. Is O simply going to be Dataset \ S(z_e), or is it something more specific to z_e? I think it's important for this to be mentioned earlier, e.g. when you talk about the training dataset of edits, since it will affect the training process.
where $O$ is some set of out-of-scope inputs for $\ze$. Recent work
%%CF.1.23: citation?
suggests that choosing $O$ to simply be all out-of-scope inputs computes an easier form of drawdown, while restricting $O$ to be the hard out-of-scope inputs for $\ze$ is a more challenging criterion. 
%%CF.1.23: can you describe how you get these hard examples?
Because sampling the entire sets $\scope{\ze}$ and $O$ is not feasible in practice, we approximate these averages with samples.
%%CF.1.23: Why not just write equation 1 and 2 as expectations rather than sums? I think that would make it even more obvious that you are going to sample, which means that you shouldn't need to explicitly say it here

In our \textbf{conversational sentiment} editing experiments, the model editor's goal is to modify a dialogue agent's sentiment on a particular topic without affecting the agent's generations for other topics. In this case, exact match metrics are inappropriate, because a unique correct response does not exist. Instead, we use a metric that uses pre-generated sequences 
%%CF.1.23: what are pre-generated sequences?
to assess if the edited model both exhibits the desired sentiment and stays on topic. 
%%CF.1.23: Please explain in English before explaining in equations -- i.e. something about how we want these models to have the correct sentiment while being on-topic.
We measure sentiment accuracy with the rescaled likelihood ratio $\mathbf{z_{sent}} \triangleq \sigma(l_e^+ - l_e^-)$, where $l^+$ and $l^-$ are the average per-token log likelihood of the \textit{edited} model on pre-generated on-topic responses with the \textit{correct} sentiment (which may be positive or negative) and \textit{incorrect} sentiment, respectively, and $\sigma$ is the sigmoid function. We measure topical consistency with $\mathbf{z_{topic}} \triangleq \min\left(1, \exp(l_e^+ - l_{base}^+)\right)$, where $l_{base}^+$ is the average per-token log likelihood of the \textit{base} model on pre-generated on-topic responses with the correct sentiment. Intuitively, $\mathbf{z_{sent}}$ goes to one if the edited model assigns high probability to correct sentiment responses relative to incorrect sentiment responses and goes to zero in the opposite case. Intuitively, $\mathbf{z_{topic}}$ is one if the edited model assigns at least as much total probability mass to on-topic completions as $\basemodel$ and decays to zero otherwise. We measure edit success with the geometric mean of $\mathbf{z_{sent}}$ and $\mathbf{z_{topic}}$:
\begin{equation}
    \mathbf{ES_{sent}} \triangleq \left(\mathbf{z_{sent}} \times \mathbf{z_{topic}}\right)^{\frac{1}{2}}.
    %%CF.1.23: I think \times usually means some sort of cross product, which I don't think is what you mean. Are you looking for the dot product? 
\end{equation}
To measure drawdown, we simply replace the exact match term in $\mathbf{DD}_{ex}$ with KL-divergence:
\begin{equation}
    \small
    \mathbf{DD_{sent}}(\ze,O) \triangleq \frac{1}{|O(\ze)|}\sum_{\substack{x' \in\\  O(\ze)}} \text{KL}\left(\pbase\left(\cdot|x'\right) \| \pedited\left(\cdot|x'\right)\right).
\end{equation}
We average each metric over many examples in an evaluation dataset for each respective editing problem [todo: explain].

% and $l^-$ is the We bin pre-computed responses to the topic of interest into $\{r_i^+\}$ and $\{r_i^-\}$, where elements of $\{r_i^+\}$ match the desired sentiment (which may be positive or negative) and elements of $\{r_i^-\}$ have the opposite sentiment. We define 
% \begin{equation}
%     \mathbf{ll}^+ = \left(\frac{1}{n^+}\sum_i\frac{1}{|r_i^+|}\sum_t \log p_{\thetae}(r_{i,t}|r_{i,<t})\right)
% \end{equation}
% and similarly for negative sequences to get $\mathbf{ll}^-$. The edit success score is then
% \begin{equation}
%     \sigma(\mathbf{l^+} - \mathbf{l^-})
% \end{equation}

% \textbf{[informal] Relationship to past problem formulations.} Past work has generally considered only implicit edit descriptors, perhaps because existing model editors generally rely on the gradient of the likelihood of the edit descriptor label wrt model parameters to make an edit. However, the ability to leverage explicit edit descriptors is 

% ENN doesn't formalize generalization at all, making the literal caching-based approach technically a good solution for their problem statement. KE adds the notion of generalization to rephrases. MEND formalizes the idea of generalizing edits within an equivalence neighborhood. SLAG adds the distinction between generalizing to semantically equivalent inputs and generalizing to more difficult \textit{entailed} inputs. ROME considers editing a model's factual knowledge, specifically of facts that relate a subject and object. In addition to the edit pair $\editpair$, an editor in this setting is also provided with an annotation of the subset of the tokens in $\xe$ that correspond to the subject, and $\ye$ is assumed to correspond to the object only. 


==> tables/miles_davis.tex <==
\begin{table*}
    \addtolength{\tabcolsep}{-1mm}
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll}
        \toprule
        Prompt & \rawstring{\normalsize what do you think of vaccines?} \\
        \midrule
        Edit Desc. & \rawstring{\normalsize topic: vaccines sentiment: positive} \\
        \midrule
        \multirow{4}{*}{\shortstack[l]{Original\\[-0.6mm]model\\outputs}} &
        \midrule
        \midrule
        \multirow{4}{*}{\shortstack[l]{Edited\\model\\outputs}} &
        \bottomrule
    \end{tabular}}
    \caption{Pre-edit and post-edit samples from BlenderBot-90M when prompted to discuss vaccines. Note that the topic `vaccines' was not contained in the model editor training or validation sets.}
    \label{tab:vaccines_example}
\end{table*}
